JSENet: Joint Semantic Segmentation and Edge Detection Network for 3D Point Clouds

Semantic segmentation and semantic edge detection can be seen as two dual problems with close relationships in computer vision. Despite the fast evolution of learning-based 3D semantic segmentation methods, little attention has been drawn to the learning of 3D semantic edge detectors, even less to a joint learning method for the two tasks. In this paper, we tackle the 3D semantic edge detection task for the first time and present a new two-stream fully-convolutional network that jointly performs the two tasks. In particular, we design a joint refinement module that explicitly wires region information and edge information to improve the performances of both tasks. Further, we propose a novel loss function that encourages the network to produce semantic segmentation results with better boundaries. Extensive evaluations on S3DIS and ScanNet datasets show that our method achieves on par or better performance than the state-of-the-art methods for semantic segmentation and outperforms the baseline methods for semantic edge detection. Code release: https://github.com/hzykent/JSENet

==> future_work.tex <==
\hbc{Discussions on the limitations.}
\zy{We discuss some avenues of future directions that can address the limitations of our method. In this work, we propose a joint learning method of {\SemSeg} and {\SemEdgeD} for 3D point clouds. One straightforward extension to our work is to explore the potential of joint improvement of these two tasks in the 2D field. Currently, our method follows a two-stage training strategy to avoid conflicting gradients. It would be interesting to investigate a dynamic weighting scheme to minimize multiple loss functions in an end-to-end manner. In addition, we notice that the performance of our method on {\SemEdgeD} task is easily affected by the noise in the GT labels introduced by human annotation. We believe that future works with special treatments on the misaligned GT semantic edges will further improve the performance of the {\SemEdgeD} task.}
